Hyperbolicity of links complements in Seifert fibered spaces

Let $\bar\gamma$ be a link in a Seifert fibered space $M$ over a hyperbolic $2$-orbifolds $\mathcal O$ that projects injectively to a filling multicurve of closed geodesics $\gamma$ in $\mathcal O.$ We prove that the complement $M_{\bar\gamma}$ of $\bar\gamma$ in $M$ admits a hyperbolic structure of finite volume and give combinatorial bounds of its volume.

==> packages.tex <==
%FONT
%\usepackage{mathpazo} % ravi -vakil text
%\usepackage{euler} % revi -vakil math


%Fundamentals
%\usepackage{pdfsync}
\usepackage{latexsym,enumitem}
\usepackage{amssymb}
\usepackage[cp850]{inputenc}
\usepackage{epsfig}
\usepackage{psfrag}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{graphics,caption}
\usepackage[all]{xy}
\usepackage{etoolbox}
\patchcmd{\quote}{\rightmargin}{\leftmargin 2em \rightmargin}{}{}
\captionsetup{width=4.7in}
%\usepackage{enumerate}
\usepackage[sort,numbers]{natbib} 
\usepackage{mathtools}



\usepackage[english]{babel}
\usepackage{comment}
\usepackage{color}
\usepackage{hyperref}


%%%%%%OPERATORS AND COMMANDS
\DeclareMathOperator{\Id}{Id} %stampa Id a testo
\DeclareMathOperator{\tr}{tr} %stampa tr a testo
\DeclareMathOperator{\diag}{diag} %stampa diag a testo
\DeclareMathOperator{\stab}{stab} %stampa stab a testo

\newcommand{\Ker}[1]{\textrm{ker}\tonde{#1}} %Ker(f)
\newcommand{\End}[2]{\textrm{End}_{#1}\tonde{#2}} %End(A,B)
\newcommand{\grado}[1]{\text{deg}(#1)} %deg(f)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%GREEK LETTERS
\let\phi\varphi
\let\deg\grado
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%COMMON USE OPERATORS
\DeclareMathOperator{\absurd}{\textrm{absurd}} %contradiction
\DeclareMathOperator{\eqdef}{\doteq\,} %definition
\DeclareMathOperator{\iffdef}{\overset{\cdot}{\iff}}  %if and only if
\newcommand{\oeq}[1]{\overset{\textrm{\tiny{#1}}}{=}}  %equality with recall
\newcommand{\f}[2]{\frac{#1}{#2}} %Fractions

%REDEFINITION OF COMMANDS
\let\epsilon\varepsilon
\let\subset\subseteq
\newcommand{\be}{\begin{equation*}}
 \newcommand{\ee}{\end{equation*}}
\newcommand{\bpf}{\begin{dimo}}
\newcommand{\epf}{\end{dimo}}
\newcommand{\bdefi}{\begin{defin}}
\newcommand{\edefi}{\end{defin}}
\newcommand{\bthm}{\begin{thm}}
\newcommand{\ethm}{\end{thm}}
\newcommand{\blem}{\begin{lem}}
\newcommand{\elem}{\end{lem}}
\newcommand{\bcor}{\begin{cor}}
\newcommand{\ecor}{\end{cor}}
\newcommand{\bfact}{\begin{f2}}
\newcommand{\efact}{\end{f2}}
\newcommand{\bprop}{\begin{prop}}
\newcommand{\eprop}{\end{prop}}
\newcommand{\bese}{\begin{ese}}
\newcommand{\eese}{\end{ese}}
\newcommand{\brem}{\begin{rem}}
\newcommand{\erem}{\end{rem}}
\newcommand{\bpfc}{\begin{dimoclaim}}
\newcommand{\epfc}{\end{dimoclaim}}
\newcommand{\eps}{\epsilon}
\newcommand{\al}{\alpha}

%ARROWS
\newcommand{\maps}{\mapsto} %arrow between objects
\newcommand{\rar}{\rightarrow} %arrow right
\newcommand{\lar}{\leftarrow} %arrow left
\newcommand{\Lar}{\,\Longleftarrow\,} %long arrow left
\newcommand{\Rar}{\,\Longrightarrow\,} %long arrow right
\newcommand{\Orar}[1]{\xrightarrow{{}_{#1}}} %long arrow right with overset
\newcommand{\Olar}[1]{\xleftarrow{{}_{#1}}} %long arrow left with overset
\newcommand{\imm}{\looparrowright}

%DIFFERENTIAL OPERATORS
\newcommand{\diff}{\mathop{}\!\mathrm{d}} %exact differential
	
%SEPARATOR AND BINARY OBJECTS
\newcommand{\divides}{\mid}									%separates
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}						%mod
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}					%norm
\newcommand{\tuple}[1]{\left\langle#1\right\rangle}					%tuple
\newcommand{\set}[1]{\left\{#1\right\}}					%set, curly brackets
\newcommand{\ceiling}[1]{\left\lceil#1\right\rceil}					%Ceiling
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}					%Floor
\newcommand{\tonde}[1]{\left(#1\right)}							%brackets
\newcommand{\quadre}[1]{\left[#1\right]}				%square brackets
\newcommand{\scalar}[2]{\left\langle #1 \,\middle |\, #2\right\rangle}	%scalar product
	
%TOPOLOGICAL AND METRICAL SPACES
\DeclareMathOperator{\interior}{int}					%Interior
\DeclareMathOperator{\cl}{cl}						%Closure
\DeclareMathOperator{\diam}{diam}					%Diameter
\newcommand{\seq}[1]{\set{#1}}					%Sequence
\newcommand{\net}[1]{\set{#1}}					%Net
\DeclareMathOperator{\opcov}{\mathcal R}			
\newcommand{\ddiscr}{d_\mathrm{discr}}				%Discrete distance
\newcommand{\chiusi}{\mathcal F}					%Closed Family
\newcommand{\T}[1]{\mathsf{{T_{#1}}}}				%Separation Axioms
\newcommand{\Num}[1]{\mathsf{{N_{#1}}}}			%Numerability Axioms
\newcommand{\Reg}[1]{\mathsf{R_{#1}}}				%Regolarity Axioms

%SETS
\newcommand{\quotient}[2]{\left.\raisebox{.1em}{$#1\!$}\middle/\raisebox{-.1em}{$#2$}\right.}
\newcommand{\backquotient}[2]{\left.\raisebox{-.1em}{$#1\,$}\middle\backslash\raisebox{.1em}{$#2$}\right.}
\newcommand{\doublequotient}[3]{\left.\raisebox{-.1em}{$#1\,$}\middle\backslash\raisebox{.1em}{$#2$}\middle/\raisebox{-.1em}{$#3$}\right.}
\newcommand{\quotientZ}[2]{\left.\raisebox{.25em}{$#1\!$}\middle/\raisebox{-.25em}{$#2$}\right.}
\DeclareMathOperator{\partsof}{\mathcal P}
	
%NUMBERS SET
\DeclareMathOperator{\emp}{\varnothing} %Known Sets, Fields and so on...
\DeclareMathOperator{\N}{\mathbb N}			%Naturals (with 0)
\DeclareMathOperator{\R}{\mathbb R}			%Reals
\DeclareMathOperator{\Q}{\mathbb Q}			%Rationals
\DeclareMathOperator{\C}{\mathbb C}			%Complexes
\DeclareMathOperator{\Z}{\mathbb Z}			%Integers
\DeclareMathOperator{\Ha}{\mathbb H}			%Hamiltonian Quaternions
\DeclareMathOperator{\I}{\mathbb I}				%Imaginary numbers
\DeclareMathOperator{\Prime}{\mathbb P}		%Prime numbers
\newcommand{\Kk}{\mathbb K}				%Base-field
\newcommand{\K}{\Bbbk}						%Field
\newcommand{\Fp}{\mathbb F_p}				%Finite field of cardinality p
\newcommand{\Fq}{\mathbb F_q}				%Finite field of cardinality q=p^n
\DeclareMathOperator{\Proj}{\mathbb P}			%Projective
\DeclareMathOperator{\Rp}{\mathbb {RP}}	        %Real Projective Space
\DeclareMathOperator{\Sph}{\mathbb S} 			%Sphere

%LIE ALGEBRAS
\newcommand{\m}{\mathfrak m}
\newcommand{\g}{\mathfrak g}
\newcommand{\h}{\mathfrak h}
\newcommand{\scal}{\mathfrak d}
\newcommand{\tri}{\mathfrak b}
\newcommand{\n}{\mathfrak n}
\newcommand{\p}{\mathfrak p}
\newcommand{\z}{\mathfrak z}
\newcommand{\symp}{\mathfrak{sp}} %sp
\newcommand{\gl}{\mathfrak{gl}}
\newcommand{\spel}{\mathfrak{sl}} %sl
\newcommand{\so}{\mathfrak{so}}
\newcommand{\ort}{\mathfrak{o}}
\newcommand{\bra}[2]{\quadre{#1,#2}} %lie bracket

%APPLICATIONS
\DeclareMathOperator{\im}{Im} %image
\DeclareMathOperator{\dom}{dom} %domain
\newcommand{\restr}{\big\lvert} %restriction

%GROUPS
\newcommand{\group}[1]{\tonde{#1,\circ_{#1}}}
\DeclareMathOperator{\id}{id} %identity map
\let \Id\id
\newcommand{\gmod}[1]{\quad \tonde{#1}} %mod 
\newcommand{\indice}[2]{\quadre{#1:#2}} %index
\newcommand{\acts}{\ \rotatebox[origin=c]{-180}{$\circlearrowright$}\ }

%FIELDS
\newcommand{\subsetk}{\underset{{}^{\cdot\cdot\cdot}}{\subset}}
\newcommand{\subsetneqk}{\underset{{}^{\cdot\cdot\cdot}}{\subsetneq}}
	
%VECTOR SPACES
\DeclareMathOperator{\mat}{\mathcal M} %matrix
\DeclareMathOperator{\rk}{rk} %rank
\DeclareMathOperator{\transpose}{^{\!\intercal}} %transpose
\DeclareMathOperator{\Endom}{End} %Endomorphism
\DeclareMathOperator{\homo}{Hom} %Homomorphism
\newcommand{\Hom}[2]{\homo\tonde{{#1},{#2}}} %Homomorphism with spaces
\DeclareMathOperator{\Sym}{Sym} %Symmetric space
\DeclareMathOperator{\Aut}{Aut} %Automorphism
\DeclareMathOperator{\Span}{span} %Span
\DeclareMathOperator{\Gr}{Gr} %Grassmannians
\DeclareMathOperator{\GL}{GL} %Invertible matrices
\setcounter{MaxMatrixCols}{20}				%Max number of matrix columns: default=10

%SHEAFS
%\newcommand{\A}{\mathscr A}
\newcommand{\B}{\mathscr B}
\newcommand{\Zq}{\mathscr Z}
\newcommand{\F}{\mathscr F}
\newcommand{\G}{\mathscr G}
\newcommand{\Os}{\mathscr O}
\newcommand{\M}{\mathscr M}
\newcommand{\Hs}{\mathscr H}
\newcommand{\coker}{\text{coker}}

%TOPOLOGY
\newcommand{\Cat}[1]{\text{cat}(#1)} %category of a space
\newcommand{\rank}[1]{\text{rank}(#1)} %rank of a space

%MANIFOLD
\newcommand{\difff}{\textrm{d}\!\!f} %differential of f
\newcommand{\defrac}[2]{\frac{\partial #1}{\partial #2}} %partial differential
\newcommand{\difrac}[2]{\frac{\diff#1}{\diff#2}} %exact differential
\newcommand{\de}[1]{\partial_{{#1}}}
\newcommand{\opar}{\overline{\partial}}
\newcommand{\diffeo}{\xrightarrow{{}_{\simeq}}} %diffeomorphism
\newcommand{\bH}{\mathbb H^3}
 \newcommand{\hyp}[1]{\quotient{\bH}{#1}}
  \newcommand{\iso}{\overset{\text{iso}}\simeq}
\newcommand{\subgroup}{\leqslant}
  \DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\dg}{deg}
\DeclareMathOperator{\Diff}{Diff}    

%SYMPLECTIC TOPOLOGY
\newcommand{\w}{\omega} %symplectic forms

%CATEGORY THEORY
\newcommand{\cat}[1]{\textbf{\textsf{#1}}} %Cat


\renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%NB: La numerazione  complessiva!

%ENVIRONMENTS
%\newenvironment{quot}
%{
%\vspace{0.7cm}
%\begin{quotation}}
%{\end{quotation}
%\vspace{0.2cm}
%}



\newenvironment{quot}
{
	\vspace{-0.2cm}
	%\begin{addmargin}[3.5em]{2.5em}}
	%{\end{addmargin}
	\vspace{0.2cm}
}



%DEFINITIONS
\theoremstyle{definition}
%\theoremstyle{definition}
\newtheorem{d1}{Definition}[section] %fa partire tutto da [section]

\newenvironment{defin}
{
	%\vspace{-0.7cm}
	\begin{quot}
		\begin{d1}
		}
		%
		{\end{d1}
	\end{quot}

	%\vspace{0.2cm}
}




%REMARKS
\theoremstyle{definition}
\newtheorem{r1}[d1]{Remark}%[section]

\newenvironment{rem}
{
	%\vspace{-0.7cm}
	\begin{quot}
		\renewcommand{\qedsymbol}{$\square$}\begin{r1}
		}
		%
		{\end{r1}
	\end{quot}
	%\vspace{0.2cm}
}

%EXERCISE
\theoremstyle{definition}
\newtheorem{e1}[d1]{Exercise}%[section]

\newenvironment{ex}
{
	%\vspace{-0.7cm}
	\begin{quot}
		\begin{e1}}
		{\end{e1}
	\end{quot}
%\vspace{0.2cm}
}

%EXAMPLE
\theoremstyle{definition}
\newtheorem{ese1}[d1]{Example}

\newenvironment{ese}
{
	%\vspace{-0.7cm}
	\begin{quot}
		\begin{ese1}
	}
	{	
		\end{ese1}
	\end{quot}
	%\vspace{0.2cm}
}

%FORMULATIONS
\theoremstyle{definition}
\newtheorem{f1}[d1]{Formulation}

%FORMULATIONS
\theoremstyle{definition}
\newtheorem{f2}[d1]{Fact}

%CONJECTURES
\theoremstyle{definition}
\newtheorem{con1}[d1]{Conjecture}


%CONJECTURES (UNLABELED)
\theoremstyle{definition}
\newtheorem*{con2}{Question}


%THEOREMS
\theoremstyle{definition}
%\theoremstyle{plain}
\newtheorem{t1}[d1]{Theorem}%[section]

\newenvironment{thm}
{
	%\vspace{-0.7cm}
	\begin{quot}
		\begin{t1}}
		{\end{t1}
	\end{quot}
	%\vspace{0.2cm}
}


%THEOREMS
\theoremstyle{definition}
%\theoremstyle{plain}
\newtheorem*{T1*}{Theorem}%[section]

\newenvironment{teor*}
{
	%\vspace{-0.7cm}
	\begin{quot}
		\begin{T1*}}
		{\end{T1*}
	\end{quot}
	%\vspace{0.2cm}
}


%DEMONSTRATIONS
\newenvironment{dimo}
{\begin{proof}[Proof]
		%$\phantom{aaaa}\\$ $\quad\,$
	}
	{\end{proof}}

\newtheorem{d10}{Definition}[section]


\newenvironment{dimoclaim}{\emph{Proof of Claim:}\;}{\hfill$\square$}



\newenvironment{dimospace}
{\begin{proof}[Proof]
		$\phantom{aaaa}\\$ $\quad\,$
	}
	{\end{proof}}

\newenvironment{sketch}
{\begin{proof}[Sketch]
		%$\phantom{aaaa}\\$ $\quad\,$
	}
	{\renewcommand{\qedsymbol}{}
	\end{proof}}
	
	%LEMMAS
	\theoremstyle{definition}
	%\theoremstyle{plain}
	\newtheorem{l1}[d1]{Lemma}%[section]
	
	\newenvironment{lem}
	{
		%\vspace{-0.7cm}
		\begin{quot}
			\begin{l1}}
			{\end{l1}
		\end{quot}
		%\vspace{0.2cm}
	}
	%PROPOSITION
	\theoremstyle{definition}
	%\theoremstyle{plain}
	\newtheorem{p1}[d1]{Proposition}%[section]
	
	\newenvironment{prop}
	{
		%\vspace{-0.7cm}
		\begin{quot}
			\begin{p1}}
			{\end{p1}
		\end{quot}
		%\vspace{0.2cm}
	}
	
	%COROLLARIES
	\theoremstyle{definition}
	%\theoremstyle{plain}
	\newtheorem{c1}[d1]{Corollary}%[section]
	
	\newenvironment{cor}
	{
		%\vspace{-0.7cm}
		\begin{quot}
			\begin{c1}}
			{\end{c1}
		\end{quot}
		%\vspace{0.2cm}
	}
	
	
	%ABSTRACT
	
		\renewenvironment{abstract}
	{\list{}{\rightmargin\leftmargin}%
		\item[\textbf{Abstract:}]\relax}
	{\endlist}
	
	
	
%THEOREMS WITHOUT NUMBER


\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
  
  \newtheorem{innercustomdef}{Definition}
\newenvironment{customdef}[1]
  {\renewcommand\theinnercustomdef{#1}\innercustomdef}
  {\endinnercustomthm}
  
  \newtheorem{innercustomcor}{Corollary}
\newenvironment{customcor}[1]
  {\renewcommand\theinnercustomcor{#1}\innercustomcor}
  {\endinnercustomthm}

  \newtheorem{innercustomprop}{Proposition}
\newenvironment{customprop}[1]
  {\renewcommand\theinnercustomprop{#1}\innercustomprop}
  {\endinnercustomthm}



 \newtheorem*{Theorem*}{Theorem}
 \newtheorem*{Proposition*}{Proposition}
 \newtheorem*{Lemma*}{Lemma}	









